An Effective Data-Driven Approach for Localizing Deep Learning Faults

Deep Learning (DL) applications are being used to solve problems in critical domains (e.g., autonomous driving or medical diagnosis systems). Thus, developers need to debug their systems to ensure that the expected behavior is delivered. However, it is hard and expensive to debug DNNs. When the failure symptoms or unsatisfied accuracies are reported after training, we lose the traceability as to which part of the DNN program is responsible for the failure. Even worse, sometimes, a deep learning program has different types of bugs. To address the challenges of debugging DNN models, we propose a novel data-driven approach that leverages model features to learn problem patterns. Our approach extracts these features, which represent semantic information of faults during DNN training. Our technique uses these features as a training dataset to learn and infer DNN fault patterns. Also, our methodology automatically links bug symptoms to their root causes, without the need for manually crafted mappings, so that developers can take the necessary steps to fix faults. We evaluate our approach using real-world and mutated models. Our results demonstrate that our technique can effectively detect and diagnose different bug types. Finally, our technique achieved better accuracy, precision, and recall than prior work for mutated models. Also, our approach achieved comparable results for real-world models in terms of accuracy and performance to the state-of-the-art.

==> Scalability.tex <==
DeepCrime support 24 operators from three empirical study. In this work, we try to make Deep4Deep support 10 operators based on our time. But Deep4Deep can support all these operators if we generate a dataset for all these operators.
Compare to SoTA:
1) DeepDiagnosis: it is a hard coding rule if the developer needs to support a new bug type. They need to develop a new rule, add it to Decision Tree, and ensure consistency.
2) DeepFD built on ML classifiers needs help finding very large datasets' correlations. 
3) Deep4Deep uses an LSTM model that can automatically find correlations insight very large datasets~\cite{}. This technical insight ensures that D4D can scale up to potentially support all bug types available in the current taxonomies~\cite{}.
